Brant-X: A Unified Physiological Signal Alignment Framework

Physiological signals serve as indispensable clues for understanding various physiological states of human bodies. Most existing works have focused on a single type of physiological signals for a range of application scenarios. However, as the body is a holistic biological system, the inherent interconnection among various physiological data should not be neglected. In particular, given the brain's role as the control center for vital activities, electroencephalogram (EEG) exhibits significant correlations with other physiological signals. Therefore, the correlation between EEG and other physiological signals holds potential to improve performance in various scenarios. Nevertheless, achieving this goal is still constrained by several challenges: the scarcity of simultaneously collected physiological data, the differences in correlations between various signals, and the correlation differences between various tasks. To address these issues, we propose a unified physiological signal alignment framework, Brant-X, to model the correlation between EEG and other signals. Our approach (1) employs the EEG foundation model to data-efficiently transfer the rich knowledge in EEG to other physiological signals, and (2) introduces the two-level alignment to fully align the semantics of EEG and other signals from different semantic scales. In the experiments, Brant-X achieves state-of-the-art performance compared with task-agnostic and task-specific baselines on various downstream tasks in diverse scenarios, including sleep stage classification, emotion recognition, freezing of gaits detection, and eye movement communication. Moreover, the analysis on the arrhythmia detection task and the visualization in case study further illustrate the effectiveness of Brant-X in the knowledge transfer from EEG to other physiological signals. The model's homepage is at https://github.com/zjunet/Brant-X/.

==> components/tables/datasets.tex <==

\begin{table*}[ht]
    \caption{A review of the public multi-type physiological datasets. 
    \small In the table, ``>0'' indicates that the dataset includes the type of signals, but we cannot provide the channel number due to access restrictions. ``-'' indicates that the dataset does not contain the signal. ``various'' indicates inconsistent sampling rates within the dataset. ``D*'' is the abbreviation of the DREAMS dataset. 
    }
    \setlength\tabcolsep{3pt}
    % \renewcommand{\arraystretch}{0.9}
    \footnotesize
    \centering
    \label{tab:datasets}






\begin{tabular}{lllcccccccccccc}
\toprule
\multirow{2}{*}{\textbf{Exp/Task}}                                              & \multirow{2}{*}{\textbf{Year}} & \multirow{2}{*}{\textbf{Dataset}}                                                  & \multirow{2}{*}{\textbf{Size}} & \multirow{2}{*}{\textbf{\#Subj.}} & \multicolumn{2}{c}{\textbf{EEG}}                                             & \multicolumn{2}{c}{\textbf{ECG}}                                       & \multicolumn{2}{c}{\textbf{EOG}}                                             & \multicolumn{2}{c}{\textbf{EMG}}                                             & \multirow{2}{*}{\textbf{Other Recordings}}                                                                                                                    & \multirow{2}{*}{\textbf{Access}}                                                                                              \\
\cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13} 
                                                                                &                                &                                                                                    &                                &                                  & \#Ch.            & Samp.                                                      & \#Ch.            & Samp.                                                & \#Ch.            & Samp.                                                      & \#Ch.            & Samp.                                                      &                                                                                                                                                               &                                                                                                                               \\
\midrule
\multirow{6}{*}{\begin{tabular}[c]{@{}l@{}}Sleep\\ Staging\end{tabular}}        & 2003                           & SHHS~\citep{quan1997sleep}                                                                               & 0.01GB                         & 120                              & 2               & 125Hz                                                      & 1               & \begin{tabular}[c]{@{}c@{}}125/\\ 250Hz\end{tabular} & 2               & 50Hz                                                       & 1               & 125Hz                                                      & \begin{tabular}[c]{@{}c@{}}Thoracic, abdominal excursions, \\ airflow, pulse oximetry, heart \\ rate, body position, ambient light\end{tabular} & \href{https://physionet.org/content/shhpsgdb/1.0.0/}{Link}                                                                    \\
\cmidrule(lr){2-15}
                                                                                & 2013                           & Sleep-EDFx~\citep{kemp2000analysis}                                                                         & 8.1GB                          & 78                               & 2               & 100 Hz                                                     & \multicolumn{2}{c}{-}                                                  & 1               & 100 Hz                                                     & 1               & 100 Hz                                                     & Airflow, rectal body temperature                                                                                                                              & \href{https://physionet.org/content/sleep-edfx/1.0.0/}{Link}                                                                  \\
\cmidrule(lr){2-15}
                                                                                & 2014                           & MASS~\citep{o2014montreal}                                                                               & no\_info                       & 200                              & 4-20           & 256Hz                                                      & \textgreater{}0 & 256Hz                                                & \textgreater{}0 & 256Hz                                                      & \textgreater{}0 & 256Hz                                                      & Respiratory effort                                                                                                                                            & \href{https://borealisdata.ca/dataverse/MASS} {\begin{tabular}[c]{@{}c@{}}Need an ethical \\ approval proof\end{tabular} }   \\
\cmidrule(lr){2-15}
                                                                                & 2015                           & ISRUC~\citep{khalighi2016isruc}                                                                              & 27GB                           & 118                              & 6               & 200Hz                                                      & 1               & 200Hz                                                & 2               & 200Hz                                                      & 3               & 200Hz                                                      & \begin{tabular}[c]{@{}c@{}}Snoring, airflow, abdominal efforts,  \\ pulse oximetry, body position\end{tabular}                                                & \href{https://sleeptight.isr.uc.pt/}{Link}                                                                   \\
\cmidrule(lr){2-15}
                                                                                & 2021                           & NCH~\citep{lee2022large}                                                                                & no\_info                       & 3673                             & \textgreater{}0 & various                                                    & \textgreater{}0 & various                                              & \textgreater{}0 & various                                                    & \textgreater{}0 & various                                                    & \begin{tabular}[c]{@{}c@{}}Airflow, respiratory effort, blood \\ oxygen saturation, end-tidal $\text{CO}_2$\end{tabular}                                                & \href{https://physionet.org/content/nch-sleep/3.1.0/} { \begin{tabular}[c]{@{}c@{}}Need request \&\\ credentialing\end{tabular} }                                                  \\
\cmidrule(lr){2-15}
                                                                                & 2022                           & HMC~\citep{alvarez2021inter}                                                                                & 15.7GB                         & 151                              & 4               & 256Hz                                                      & 1               & 256Hz                                                & 2               & 256Hz                                                      & 1               & 256Hz                                                      & -                                                                                                                                                             & \href{https://physionet.org/content/hmc-sleep-staging/1.1/}{Link}                                                                  \\
\midrule
\begin{tabular}[c]{@{}l@{}}Cyclic \\ Alternating \\ Pattern\end{tabular}        & 2012                           & CAP~\citep{terzano2002atlas}                                                                                & 40.1GB                         & 108                              & 3               & 512Hz                                                      & 1               & 512Hz                                                & 2               & 512Hz                                                      & 2               & 512Hz                                                      & \begin{tabular}[c]{@{}c@{}}Airflow, abdominal and thoracic \\ effort and $\text{SaO}_2$\end{tabular}                                                                    & \href{https://physionet.org/content/capslpdb/1.0.0/}{Link}                                                                   \\
\midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Sleep \\ Apnea\end{tabular}}         & 1999                           & \begin{tabular}[c]{@{}l@{}}MIT-BIH \\ PSG~\citep{ichimaru1999development} \end{tabular}                             & 0.6GB                          & 18                               & 1               & 250Hz                                                      & 1               & 250Hz                                                & 1               & 250Hz                                                      & 1               & 250Hz                                                      & \begin{tabular}[c]{@{}c@{}}Blood pressure, respiration, cardiac \\ stroke volume, earlobe oximetry\end{tabular}                                               & \href{https://physionet.org/content/slpdb/1.0.0/}{Link}                                                                  \\
\cmidrule(lr){2-15}
& 2007                           & UCDDB~\citep{goldberger2000physiobank}                                                                              & 1.3GB                          & 25                               & 2               & 128Hz                                                      & 1               & 128Hz                                                & 2               & 128Hz                                                      & 1               & 128Hz                                                      & \begin{tabular}[c]{@{}c@{}}Airflow, ribcage movements, \\ abdomen movements, oxygen \\ saturation, snoring, body position\end{tabular}                        & \href{https://physionet.org/content/ucddb/1.0.0/}{Link}                                                                   \\
\midrule
\multirow{8}{*}{\begin{tabular}[c]{@{}l@{}}Sleep\\ (DREA- \\MS)~\citep{devuyst2005dreams}\end{tabular}}       & \multirow{8}{*}{2005}          & D* Subjects                                                                        & 1.1GB                          & 20                               & 3               & 200Hz                                                      & \multicolumn{2}{c}{-}                                                  & 2               & 200Hz                                                      & 1               & 200Hz                                                      & -                                                                                                                                                             & \multirow{8}{*}{ \href{https://zenodo.org/records/2650142}{Link}  }                                                 \\
\cmidrule(lr){3-14}
&                                & D* Patients                                                                        & 1.7GB                          & 27                               & 3               & 200Hz                                                      & \multicolumn{2}{c}{-}                                                  & 2               & 200Hz                                                      & 1               & 200Hz                                                      & -                                                                                                                                                             &                                                                                                                               \\
\cmidrule(lr){3-14}
&                                & D* Artifacts                                                                       & 0.05GB                         & 20                               & 3               & \begin{tabular}[c]{@{}c@{}}200/\\ 100/\\ 50Hz\end{tabular} & \multicolumn{2}{c}{-}                                                  & 2               & \begin{tabular}[c]{@{}c@{}}200/\\ 100/\\ 50Hz\end{tabular} & 1               & \begin{tabular}[c]{@{}c@{}}200/\\ 100/\\ 50Hz\end{tabular} & -                                                                                                                                                             &                                                                                                                               \\
\cmidrule(lr){3-14}
&                                & \begin{tabular}[c]{@{}l@{}}D* Sleep \\ Spindles\end{tabular}                       & 0.05GB                         & 8                                & 3               & \begin{tabular}[c]{@{}c@{}}200/\\ 100/\\ 50Hz\end{tabular} & \multicolumn{2}{c}{-}                                                  & 2               & \begin{tabular}[c]{@{}c@{}}200/\\ 100/\\ 50Hz\end{tabular} & 1               & \begin{tabular}[c]{@{}c@{}}200/\\ 100/\\ 50Hz\end{tabular} & -                                                                                                                                                             &                                                                                                                               \\
\cmidrule(lr){3-14}
&                                & \begin{tabular}[c]{@{}l@{}}D* K-\\ complexes\end{tabular}                          & 0.05GB                         & 10                               & 3               & 200Hz                                                      & \multicolumn{2}{c}{-}                                                  & 2               & 200Hz                                                      & 1               & 200Hz                                                      & -                                                                                                                                                             &                                                                                                                               \\
\cmidrule(lr){3-14}
&                                & D* REMs                                                                            & 0.04GB                         & 9                                & 3               & 200Hz                                                      & \multicolumn{2}{c}{-}                                                  & 2               & 200Hz                                                      & 1               & 200Hz                                                      & -                                                                                                                                                             &                                                                                                                               \\
\cmidrule(lr){3-14}
&                                & D* PLMs                                                                            & 0.6GB                          & 10                               & 3               & \begin{tabular}[c]{@{}c@{}}200/\\ 50Hz\end{tabular}      & \multicolumn{2}{c}{-}                                                  & 2               & \begin{tabular}[c]{@{}c@{}}200/\\ 50Hz\end{tabular}      & 1               & \begin{tabular}[c]{@{}c@{}}200/\\ 50Hz\end{tabular}      & -                                                                                                                                                             &                                                                                                                               \\
\cmidrule(lr){3-14}
&                                & D* Apnea                                                                           & 0.8GB                          & 12                               & 3               & 200Hz                                                      & 1               & 200Hz                                                & 2               & 200Hz                                                      & 1               & 200Hz                                                      & \begin{tabular}[c]{@{}c@{}}Air flow, abdominal and thoracic \\ inductive plethysmography\end{tabular}                                                         &                                                                                                                               \\
\midrule
\begin{tabular}[c]{@{}l@{}}Electrical \\ Stimulation\end{tabular}               & 2021                           & \begin{tabular}[c]{@{}l@{}}Gebodh \\ et al.~\citep{gebodh2021dataset}\end{tabular}                           & 65GB                           & 20                               & 32              & \begin{tabular}[c]{@{}c@{}}1000/\\ 2000Hz\end{tabular}     & 1               & 1000Hz                                               & 1               & 1000Hz                                                     & \multicolumn{2}{c}{-}                                                        & \begin{tabular}[c]{@{}c@{}}Behavioral vigilance and \\ alertness metrics\end{tabular}                                                                         & \href{https://zenodo.org/records/4456079}{Link}                                                                \\
\midrule
\begin{tabular}[c]{@{}l@{}}Freezing \\ of Gaits\end{tabular}                    & 2022                           & \begin{tabular}[c]{@{}l@{}}Zhang \\ et al.~\citep{zhang2022multimodal}\end{tabular}                            & 1.6GB                          & 12                               & 25              & 1000Hz                                                     & \multicolumn{2}{c}{-}                                                  & \multicolumn{2}{c}{-}                                                        & 3               & 1000Hz                                                     & Gait acceleration, skin conductance                                                                                                                           & \href{https://data.mendeley.com/datasets/r8gmbtv7w2/3}{Link}                                                                   \\
\midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Emotion \\ Recognition\end{tabular}} & 2012                           & DEAP~\citep{koelstra2011deap}                                                                               & 2.7GB                          & 32                               & 32              & 512Hz                                                      & \multicolumn{2}{c}{-}                                                  & 4               & 512Hz                                                      & 4               & 512Hz                                                      & \begin{tabular}[c]{@{}c@{}}Video, respiration, plethysmograph, \\ temperature\end{tabular}                                                                    & \href{https://www.eecs.qmul.ac.uk/mmv/datasets/deap/index.html}{Link}                                                                  \\
\cmidrule(lr){2-15}
                                                                                & 2017                           & DREAMER~\citep{katsigiannis2017dreamer}                                                                            & 0.5GB                          & 23                               & 14              & 128Hz                                                      & 2               & 256Hz                                                & \multicolumn{2}{c}{-}                                                        & \multicolumn{2}{c}{-}                                                        & Video                                                                                                                                                         & \href{https://zenodo.org/records/546113}{ \begin{tabular}[c]{@{}c@{}}Need \\ request\end{tabular} }                                                                      \\
\midrule
\begin{tabular}[c]{@{}l@{}}Stress and \\ Affect \\ Detection\end{tabular}       & 2018                           & WESAD~\citep{schmidt2018introducing}                                                                              & 17GB                           & 15                               & \multicolumn{2}{c}{-}                                                        & 1               & 700Hz                                                & \multicolumn{2}{c}{-}                                                        & 1               & 700Hz                                                      & \begin{tabular}[c]{@{}c@{}}Acceleration, respiration, \\ electrodermal activity, body \\ temperatur, blood volume pulse\end{tabular}                          & \href{https://complexity.cecs.ucf.edu/wesad-wearable-stress-and-affect-detection/}{Link}                                                                  \\
\midrule
\begin{tabular}[c]{@{}l@{}}Eye \\ Movement\end{tabular}                         & 2021                           & \begin{tabular}[c]{@{}l@{}}Jaramillo-\\ Gonzalez \\ et al.~\citep{jaramillo2021dataset}\end{tabular}            & 3.9GB                          & 4                                & \textgreater{}0 & 500Hz                                                      & \multicolumn{2}{c}{-}                                                  & \textgreater{}0 & 500Hz                                                      & \multicolumn{2}{c}{-}                                                        & -                                                                                                                                               & \href{https://zenodo.org/record/4002038}{Link}                                                                \\
\midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Motor \\ Imagery\end{tabular}}       & \multirow{3}{*}{2008}          & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}BCI Com-\\ petition \\ IV~\citep{blankertz2006bci}\end{tabular}} & \multirow{3}{*}{3.2GB}         & 7                                & 64              & 1000Hz                                                     & \multicolumn{2}{c}{-}                                                  & \multicolumn{2}{c}{-}                                                        & \multicolumn{2}{c}{-}                                                        & -                                                                                                                                               & \multirow{3}{*}{ \href{https://www.bbci.de/competition/iv/}{Link}  }                                                 \\
\cmidrule(lr){5-14}
                                                                                &                                &                                                                                    &                                & 9                                & 22              & 250Hz                                                      & \multicolumn{2}{c}{-}                                                  & 3               & 250Hz                                                      & \multicolumn{2}{c}{-}                                                        & -                                                                                                                                               &                                                                                                                               \\
\cmidrule(lr){5-14}
&                                &                                                                                    &                                & 9                                & 3               & 250Hz                                                      & \multicolumn{2}{c}{-}                                                  & 3               & 250Hz                                                      & \multicolumn{2}{c}{-}                                                        & -                                                                                                                                               &                                                                                                                               \\
\cmidrule(lr){2-15}
                                                                                & 2020                           & BNCI                                                                               & \multicolumn{11}{c}{Multiple datasets. Please refer to the link for detailed information.}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    & \href{https://bnci-horizon-2020.eu/database/data-sets}{Link}       \\                                                           
\bottomrule
\end{tabular}





\end{table*}


==> components/tables/datasets_nolink.tex <==

\begin{table*}[ht]
    \caption{A review of the public multi-type physiological datasets. 
    \small In the table, ``>0'' indicates that the dataset includes the type of signals, but we cannot provide the channel number due to access restrictions. ``-'' indicates that the dataset does not contain the signal. ``varying'' indicates inconsistent sampling rates within the dataset. ``D*'' is the abbreviation of the DREAMS dataset. 
    }
    \setlength\tabcolsep{3.3pt}
    \renewcommand{\arraystretch}{0.9}
    \footnotesize
    \centering
    \label{tab:datasets}






\begin{tabular}{lllcccccccccccc}
\toprule
\multirow{2}{*}{\textbf{Exp/Task}}                                              & \multirow{2}{*}{\textbf{Year}} & \multirow{2}{*}{\textbf{Dataset}}                                                  & \multirow{2}{*}{\textbf{Size}} & \multirow{2}{*}{\textbf{\#Subj}} & \multicolumn{2}{c}{\textbf{EEG}}                                             & \multicolumn{2}{c}{\textbf{ECG}}                                       & \multicolumn{2}{c}{\textbf{EOG}}                                             & \multicolumn{2}{c}{\textbf{EMG}}                                             & \multirow{2}{*}{\textbf{Other Recordings}}                                                                                                                    & \multirow{2}{*}{\textbf{Access}}                                                                                              \\
\cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13} 
                                                                                &                                &                                                                                    &                                &                                  & \#Ch            & Samp.                                                      & \#Ch            & Samp.                                                & \#Ch            & Samp.                                                      & \#Ch            & Samp.                                                      &                                                                                                                                                               &                                                                                                                               \\
\midrule
\multirow{6}{*}{\begin{tabular}[c]{@{}l@{}}Sleep\\ Staging\end{tabular}}        & 2003                           & SHHS                                                                               & 0.01GB                         & 120                              & 2               & 125Hz                                                      & 1               & \begin{tabular}[c]{@{}c@{}}125/\\ 250Hz\end{tabular} & 2               & 50Hz                                                       & 1               & 125Hz                                                      & \begin{tabular}[c]{@{}c@{}}Thoracic, abdominal excursions, \\ airflow, pulse oximetry, heart \\ rate, body position, ambient light\end{tabular} & \begin{tabular}[c]{@{}c@{}}Download \\ directly\end{tabular}                                                                  \\
\cmidrule(lr){2-15}
                                                                                & 2013                           & Sleep-EDFx                                                                         & 8.1GB                          & 78                               & 2               & 100 Hz                                                     & \multicolumn{2}{c}{-}                                                  & 1               & 100 Hz                                                     & 1               & 100 Hz                                                     & Airflow, rectal body temperature                                                                                                                              & \begin{tabular}[c]{@{}c@{}}Download \\ directly\end{tabular}                                                                  \\
\cmidrule(lr){2-15}
                                                                                & 2014                           & MASS                                                                               & no\_info                       & 200                              & 45402           & 256Hz                                                      & \textgreater{}0 & 256Hz                                                & \textgreater{}0 & 256Hz                                                      & \textgreater{}0 & 256Hz                                                      & Respiratory effort                                                                                                                                            & \begin{tabular}[c]{@{}c@{}}Need an ethical \\ approval proof\end{tabular} \\
\cmidrule(lr){2-15}
                                                                                & 2015                           & ISRUC                                                                              & 27GB                           & 118                              & 6               & 200Hz                                                      & 1               & 200Hz                                                & 2               & 200Hz                                                      & 3               & 200Hz                                                      & \begin{tabular}[c]{@{}c@{}}Snoring, airflow, abdominal efforts,  \\ pulse oximetry, body position\end{tabular}                                                & \begin{tabular}[c]{@{}c@{}}Download \\ directly\end{tabular}                                                                  \\
\cmidrule(lr){2-15}
                                                                                & 2021                           & NCH                                                                                & no\_info                       & 3673                             & \textgreater{}0 & varying                                                    & \textgreater{}0 & varying                                              & \textgreater{}0 & varying                                                    & \textgreater{}0 & varying                                                    & \begin{tabular}[c]{@{}c@{}}Airflow, respiratory effort, blood \\ oxygen saturation, end-tidal CO2\end{tabular}                                                & \begin{tabular}[c]{@{}c@{}}Need request \&\\ credentialing\end{tabular}                                                  \\
\cmidrule(lr){2-15}
                                                                                & 2022                           & HMC                                                                                & 15.7GB                         & 151                              & 4               & 256Hz                                                      & 1               & 256Hz                                                & 2               & 256Hz                                                      & 1               & 256Hz                                                      & -                                                                                                                                                             & \begin{tabular}[c]{@{}c@{}}Download \\ directly\end{tabular}                                                                  \\
\midrule
\begin{tabular}[c]{@{}l@{}}Cyclic \\ Alternating \\ Pattern\end{tabular}        & 2012                           & CAP                                                                                & 40.1GB                         & 108                              & 3               & 512Hz                                                      & 1               & 512Hz                                                & 2               & 512Hz                                                      & 2               & 512Hz                                                      & \begin{tabular}[c]{@{}c@{}}Airflow, abdominal and thoracic \\ effort and SaO2\end{tabular}                                                                    & \begin{tabular}[c]{@{}c@{}}Download \\ directly\end{tabular}                                                                  \\
\midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Sleep \\ Apnea\end{tabular}}         & 1999                           & \begin{tabular}[c]{@{}l@{}}MIT-BIH \\ PSG\end{tabular}                             & 0.6GB                          & 18                               & 1               & 250Hz                                                      & 1               & 250Hz                                                & 1               & 250Hz                                                      & 1               & 250Hz                                                      & \begin{tabular}[c]{@{}c@{}}Blood pressure, respiration, cardiac \\ stroke volume, earlobe oximetry\end{tabular}                                               & \begin{tabular}[c]{@{}c@{}}Download \\ directly\end{tabular}                                                                  \\
\cmidrule(lr){2-15}
& 2007                           & UCDDB                                                                              & 1.3GB                          & 25                               & 2               & 128Hz                                                      & 1               & 128Hz                                                & 2               & 128Hz                                                      & 1               & 128Hz                                                      & \begin{tabular}[c]{@{}c@{}}Airflow, ribcage movements, \\ abdomen movements, oxygen \\ saturation, snoring, body position\end{tabular}                        & \begin{tabular}[c]{@{}c@{}}Download \\ directly\end{tabular}                                                                  \\
\midrule
\multirow{8}{*}{\begin{tabular}[c]{@{}l@{}}Sleep\\ (DREAMS)\end{tabular}}       & \multirow{8}{*}{2005}          & D* Subjects                                                                        & 1.1GB                          & 20                               & 3               & 200Hz                                                      & \multicolumn{2}{c}{-}                                                  & 2               & 200Hz                                                      & 1               & 200Hz                                                      & -                                                                                                                                                             & \multirow{8}{*}{\begin{tabular}[c]{@{}c@{}}Download \\ directly\end{tabular}}                                                 \\
\cmidrule(lr){3-14}
&                                & D* Patients                                                                        & 1.7GB                          & 27                               & 3               & 200Hz                                                      & \multicolumn{2}{c}{-}                                                  & 2               & 200Hz                                                      & 1               & 200Hz                                                      & -                                                                                                                                                             &                                                                                                                               \\
\cmidrule(lr){3-14}
&                                & D* Artifacts                                                                       & 0.05GB                         & 20                               & 3               & \begin{tabular}[c]{@{}c@{}}200/\\ 100/\\ 50Hz\end{tabular} & \multicolumn{2}{c}{-}                                                  & 2               & \begin{tabular}[c]{@{}c@{}}200/\\ 100/\\ 50Hz\end{tabular} & 1               & \begin{tabular}[c]{@{}c@{}}200/\\ 100/\\ 50Hz\end{tabular} & -                                                                                                                                                             &                                                                                                                               \\
\cmidrule(lr){3-14}
&                                & \begin{tabular}[c]{@{}l@{}}D* Sleep \\ Spindles\end{tabular}                       & 0.05GB                         & 8                                & 3               & \begin{tabular}[c]{@{}c@{}}200/\\ 100/\\ 50Hz\end{tabular} & \multicolumn{2}{c}{-}                                                  & 2               & \begin{tabular}[c]{@{}c@{}}200/\\ 100/\\ 50Hz\end{tabular} & 1               & \begin{tabular}[c]{@{}c@{}}200/\\ 100/\\ 50Hz\end{tabular} & -                                                                                                                                                             &                                                                                                                               \\
\cmidrule(lr){3-14}
&                                & \begin{tabular}[c]{@{}l@{}}D* K-\\ complexes\end{tabular}                          & 0.05GB                         & 10                               & 3               & 200Hz                                                      & \multicolumn{2}{c}{-}                                                  & 2               & 200Hz                                                      & 1               & 200Hz                                                      & -                                                                                                                                                             &                                                                                                                               \\
\cmidrule(lr){3-14}
&                                & D* REMs                                                                            & 0.04GB                         & 9                                & 3               & 200Hz                                                      & \multicolumn{2}{c}{-}                                                  & 2               & 200Hz                                                      & 1               & 200Hz                                                      & -                                                                                                                                                             &                                                                                                                               \\
\cmidrule(lr){3-14}
&                                & D* PLMs                                                                            & 0.6GB                          & 10                               & 3               & \begin{tabular}[c]{@{}c@{}}200/\\ 50Hz\end{tabular}      & \multicolumn{2}{c}{-}                                                  & 2               & \begin{tabular}[c]{@{}c@{}}200/\\ 50Hz\end{tabular}      & 1               & \begin{tabular}[c]{@{}c@{}}200/\\ 50Hz\end{tabular}      & -                                                                                                                                                             &                                                                                                                               \\
\cmidrule(lr){3-14}
&                                & D* Apnea                                                                           & 0.8GB                          & 12                               & 3               & 200Hz                                                      & 1               & 200Hz                                                & 2               & 200Hz                                                      & 1               & 200Hz                                                      & \begin{tabular}[c]{@{}c@{}}Air flow, abdominal and thoracic \\ inductive plethysmography\end{tabular}                                                         &                                                                                                                               \\
\midrule
\begin{tabular}[c]{@{}l@{}}Electrical \\ Stimulation\end{tabular}               & 2021                           & \begin{tabular}[c]{@{}l@{}}Gebodh \\ et al.\end{tabular}                           & 65GB                           & 20                               & 32              & \begin{tabular}[c]{@{}c@{}}1000/\\ 2000Hz\end{tabular}     & 1               & 1000Hz                                               & 1               & 1000Hz                                                     & \multicolumn{2}{c}{-}                                                        & \begin{tabular}[c]{@{}c@{}}Behavioral vigilance and \\ alertness metrics\end{tabular}                                                                         & \begin{tabular}[c]{@{}c@{}}Download \\ directly\end{tabular}                                                                  \\
\midrule
\begin{tabular}[c]{@{}l@{}}Freezing \\ of Gaits\end{tabular}                    & 2022                           & \begin{tabular}[c]{@{}l@{}}Zhang \\ et al.\end{tabular}                            & 1.6GB                          & 12                               & 25              & 1000Hz                                                     & \multicolumn{2}{c}{-}                                                  & \multicolumn{2}{c}{-}                                                        & 3               & 1000Hz                                                     & Gait acceleration, skin conductance                                                                                                                           & \begin{tabular}[c]{@{}c@{}}Download \\ directly\end{tabular}                                                                  \\
\midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Emotion \\ Recognition\end{tabular}} & 2012                           & DEAP                                                                               & 2.7GB                          & 32                               & 32              & 512Hz                                                      & \multicolumn{2}{c}{-}                                                  & 4               & 512Hz                                                      & 4               & 512Hz                                                      & \begin{tabular}[c]{@{}c@{}}Video, respiration, plethysmograph, \\ temperature\end{tabular}                                                                    & \begin{tabular}[c]{@{}c@{}}Download \\ directly\end{tabular}                                                                  \\
\cmidrule(lr){2-15}
                                                                                & 2017                           & DREAMER                                                                            & 0.5GB                          & 23                               & 14              & 128Hz                                                      & 2               & 256Hz                                                & \multicolumn{2}{c}{-}                                                        & \multicolumn{2}{c}{-}                                                        & Video                                                                                                                                                         & \begin{tabular}[c]{@{}c@{}}Need \\ request\end{tabular}                                                                       \\
\midrule
\begin{tabular}[c]{@{}l@{}}Stress and \\ Affect \\ Detection\end{tabular}       & 2018                           & WESAD                                                                              & 17GB                           & 15                               & \multicolumn{2}{c}{-}                                                        & 1               & 700Hz                                                & \multicolumn{2}{c}{-}                                                        & 1               & 700Hz                                                      & \begin{tabular}[c]{@{}c@{}}Acceleration, respiration, \\ electrodermal activity, body \\ temperatur, blood volume pulse\end{tabular}                          & \begin{tabular}[c]{@{}c@{}}Download \\ directly\end{tabular}                                                                  \\
\midrule
\begin{tabular}[c]{@{}l@{}}Eye \\ Movement\end{tabular}                         & 2021                           & \begin{tabular}[c]{@{}l@{}}Jaramillo-\\ Gonzalez \\ et al.\end{tabular}            & 3.9GB                          & 4                                & \textgreater{}0 & 500Hz                                                      & \multicolumn{2}{c}{-}                                                  & \textgreater{}0 & 500Hz                                                      & \multicolumn{2}{c}{-}                                                        & -                                                                                                                                               & \begin{tabular}[c]{@{}c@{}}Download \\ directly\end{tabular}                                                                  \\
\midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Motor \\ Imagery\end{tabular}}       & \multirow{3}{*}{2008}          & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}BCI Com-\\ petition \\ IV\end{tabular}} & \multirow{3}{*}{0.5GB}         & 7                                & 64              & 1000Hz                                                     & \multicolumn{2}{c}{-}                                                  & \multicolumn{2}{c}{-}                                                        & \multicolumn{2}{c}{-}                                                        & -                                                                                                                                               & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Download \\ directly\end{tabular}}                                                 \\
\cmidrule(lr){5-14}
                                                                                &                                &                                                                                    &                                & 9                                & 22              & 250Hz                                                      & \multicolumn{2}{c}{-}                                                  & 3               & 250Hz                                                      & \multicolumn{2}{c}{-}                                                        & -                                                                                                                                               &                                                                                                                               \\
\cmidrule(lr){5-14}
&                                &                                                                                    &                                & 9                                & 3               & 250Hz                                                      & \multicolumn{2}{c}{-}                                                  & 3               & 250Hz                                                      & \multicolumn{2}{c}{-}                                                        & -                                                                                                                                               &                                                                                                                               \\
\cmidrule(lr){2-15}
                                                                                & 2020                           & BNCI                                                                               & \multicolumn{11}{c}{multiple datasets}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    & \begin{tabular}[c]{@{}c@{}}Download \\ directly\end{tabular}       \\                                                           
\bottomrule
\end{tabular}





\end{table*}

